Leveraging Continuously Differentiable Activation Functions for Learning in Quantized Noisy Environments

Real-world analog systems intrinsically suffer from noise that can impede model convergence and accuracy on a variety of deep learning models. We demonstrate that differentiable activations like GELU and SiLU enable robust propagation of gradients which help to mitigate analog quantization error that is ubiquitous to all analog systems. We perform analysis and training of convolutional, linear, and transformer networks in the presence of quantized noise. Here, we are able to demonstrate that continuously differentiable activation functions are significantly more noise resilient over conventional rectified activations. As in the case of ReLU, the error in gradients are 100x higher than those in GELU near zero. Our findings provide guidance for selecting appropriate activations to realize performant and reliable hardware implementations across several machine learning domains such as computer vision, signal processing, and beyond. Code available at: \href{https://github.com/Vivswan/GeLUReLUInterpolation}{https://github.com/Vivswan/GeLUReLUInterpolation}.}

==> sections/11-IEEEBio.tex <==
% \newpage
\vspace{-40mm}
\begin{IEEEbiographynophoto}{Vivswan Shah} received the B.S. degree in Computer Science and Physics from Illinois College in 2018. From 2018 to 2019, he was a research assistant in Reinforcement Learning and Computational Biology groups, focusing on machine learning algorithms and clustering techniques. He is currently pursuing a Ph.D. in Machine Learning Systems at the University of Pittsburgh. His dissertation focuses on real-time distributed deep learning over heterogeneous systems. He has worked with organizations including Amazon and Google X, with research interests spanning generative AI, large language models, computer vision, and photonic AI accelerators. 
\end{IEEEbiographynophoto}

\vspace{-40mm}
\begin{IEEEbiographynophoto}{Nathan Youngblood} (Member, IEEE) received the B.S. degree in physics from Bethel University, St. Paul, MN, USA in 2011 and the Ph.D. degree in electrical engineering from the University of Minnesota, Minneapolis, MN, USA in 2016 where he was involved in the integration of 2-D materials with silicon photonics for optoelectronic applications. After postdoctoral training at the University of Oxford, Oxford, UK, he joined the Department of Electrical and Computer Engineering at the University of Pittsburgh, Pittsburgh, PA, USA in 2019. His research interests include integrated photonics, high-speed optoelectronics, artificial intelligence, and novel computing methods with light.

\end{IEEEbiographynophoto}


==> sections/8-Acknowledgement.tex <==
\section{Acknowledgement}
This research was supported in part by the University of Pittsburgh Center for Research Computing, RRID:SCR\_022735, through the resources provided. Specifically, this work used the H2P cluster, which is supported by NSF award number OAC-2117681.

==> sections/9-ImpactStatements.tex <==
\section{Societal Impacts}
This work aims to advance machine learning capabilities for real-world applications. Like most technical advances, it has potential for both beneficial and harmful uses, depending on the context. We encourage thoughtful consideration of intended applications to help ensure methods are applied ethically, particularly for safety-critical systems where reliability and robustness are paramount. Overall, we believe the insights provided will primarily further progress towards safe, reliable, and responsible AI.
